Cine-AI: Generating Video Game Cutscenes in the Style of Human Directors

Cutscenes form an integral part of many video games, but their creation is costly, time-consuming, and requires skills that many game developers lack. While AI has been leveraged to semi-automate cutscene production, the results typically lack the internal consistency and uniformity in style that is characteristic of professional human directors. We overcome this shortcoming with Cine-AI, an open-source procedural cinematography toolset capable of generating in-game cutscenes in the style of eminent human directors. Implemented in the popular game engine Unity, Cine-AI features a novel timeline and storyboard interface for design-time manipulation, combined with runtime cinematography automation. Via two user studies, each employing quantitative and qualitative measures, we demonstrate that Cine-AI generates cutscenes that people correctly associate with a target director, while providing above-average usability. Our director imitation dataset is publicly available, and can be extended by users and film enthusiasts.

==> sections/system_old.tex <==
\section{\ProjectName{} System and User Interface}
\label{section:system}

We next describe the processes and user interfaces through which \ProjectName{} accomplishes the procedural generation of in-game cutscenes in a target director's style, with an emphasis on the design-time user interaction. The following subsections provide detail on one or multiple design-time (sub-)processes, as illustrated and referenced in Figure \ref{fig:activityuml}. In the last subsection, we elaborate on the system's runtime support for dynamic in-game cutscenes. 

In order to support \ProjectName{}'s straight-forward application in real-life game production, we have implemented the system in the popular Unity game engine. As an additional advantage, the Unity Editor provides an extensive set of tools for cutscene production, such as sequence and timeline editors, as well as immediate GUI libraries. 

%The interaction and processing steps of \ProjectName{} can be summarized as follows, with more implementation details and design rationale provided in the sections below.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig/Cine-AI_flowchart.pdf}
  \caption{UML Activity diagram of \ProjectName{}'s design-time (sub-) processes (\textbf{rounded rectangles} - actions, \textbf{diamonds} - conditions, \textbf{circles} - start/end of overall or sub-process). \textbf{Blue} components require user interaction, \textbf{green} ones are fully automated. Numbers above each component refer to the subsection in which it is described in detail.}\label{fig:activityuml}
\end{figure}

%\begin{itemize}
%\item Users are required to input the director style data obtained by the process described in Sec.~\ref{section:data_annotation}. 
%\item Processing this data, the system defines the cinematography rules to abide by in order to generate camera behaviour in the style of the director. 

%\item \textit{Shot markers} are used to define cuts and transitions. The user places the markers at desired position on a timeline view.

%\item Users are also given a set of parameters to tweak the behaviour of the toolset depending on their project needs. These parameters mostly define 3D scene specific settings like camera distances, allowed field-of-view ranges and geometry analysis.

%\item \ProjectName{} collects static collision data from the cutscene by calculating scene proxies, 3D volumes that are used to define the boundaries of the cutscene.

%\item Users can simulate all or specific shot markers over the cutscene. Simulation of a marker triggers the system to choose a specific cinematography techniques for the marker's point in the timeline.  A new camera behaviour, including the camera placement, angle, path, alignment and lens parameters is calculated based on the chosen techniques. 

%\item After all shot markers are simulated, the calculated data is presented to the user in the form of a storyboard, where each marker will correspond to a single node, along with a preview of the calculated shot. Users can individually tweak the calculated data or re-simulate completely if they desire.

%\item After a final scene composition is achieved, users simply trigger their cutscenes during the game and notify \ProjectName{}'s event system, which controls all camera behaviour in runtime based on the data that was calculated during design-time. 
%\end{itemize}

\subsection{Director Data Input \& Processing}
\label{sec:system_data}

The user initialises \ProjectName{} by inputting a director imitation dataset, obtained through the process described in Sec.~\ref{section:data_annotation}. As a prerequisite to deciding which cinematography rules to abide by to generate camera behaviour in the style of the encoded director, \ProjectName{} calculates the conditional probabilities of each technique $t$ to occur within a category $C$ as
%In order to choose a cinematography technique for a shot marker in the timeline,
%, coded during the director analysis stage. When a director's data is imported,
\begin{equation}
p(t|C) = 
\begin{cases} f_t / \sum\limits_{t^\prime\in\ C}f_{t^\prime} &\text{, if } t\in C\\
0&\text{, otherwise.} 
\end{cases}
\end{equation}
This processing step relies on $f_t$, the total frequency of a technique observed over all clips, as comprised in the dataset.

\iffalse
\begin{figure}[ht]
  \centering
  \includegraphics[width=3in]{fig/directorData2.png}
  \caption{\textcolor{red}{Remove? }Categorized director data showing default (${P}_x$) for the cinematography techniques.}\label{fig:dirdata}
\end{figure}
\fi 

\subsection{Defining Shot Markers}
The user defines shot markers in the Unity Editor animation timeline (Figure \ref{fig:markers_timeline}) to indicate at which time \ProjectName{} should insert cuts and transitions into the cutscene (Supplementary Video, 01:08). For each individual marker, the user can specify dramatisation and pace values, as well as which game object(s) the camera should focus on (Figure \ref{fig:markers_settings}) .
%By evaluating all markers,  \ProjectName{} will decide on a new cinematography technique per marker, thus a new camera framing, movement and transition, resulting in a cut. Each marker will correspond to a node in the generated storyboard, which will be further explained later.

\begin{figure}[ht]
  \subcaptionbox{Shot markers in Unity Editor animation timeline\label{fig:markers_timeline}}{\includegraphics[height=1.75in]{fig/markers.png} }\hfill%
  \subcaptionbox{Example marker settings\label{fig:markers_settings}}{\includegraphics[height=1.75in]{fig/marker_settings.png}}%
  \caption{Shot marker user interface. The user defines markers (\textbf{grey drop shapes}) in the Unity Editor animation timeline (a). For each marker, they can then set the camera target, and specify a desired transition dramatisation and pace.}
  \label{fig:markers}
\end{figure}

\subsection{Scene Proxies and Collision Information}
\label{sec:system_proxies}
%\ProjectName{} collects static collision data from the cutscene by calculating scene proxies, 3D volumes that are used to define the boundaries of the cutscene.

To prevent camera clipping and realise collision-free camera paths, \ProjectName{} must obtain 3D collision information from the scene geometry. This calculation is expensive, but a cutscene is typically only set in a small part of the game world (Figure \ref{fig:proxies_initial}). For increased efficiency, \ProjectName{} requires the user to set up scene proxies, i.e. 3D volumes that delimit the area in which the cutscene takes place, and for which collision information is required (Supplementary Video, 01:28).
%\ProjectName{}'s interface provides parameters to adjust proxy settings per cutscene.

\iffalse
\begin{figure}[ht]
  \centering
  \includegraphics[width=4.0in]{fig/proxySettings.png}
  \caption{Exposed proxy parameters allow the users to compute proxy cells with an accuracy of their choice.}\label{fig:proxySettings}
\end{figure}
%These settings define the boundaries of the proxies and their collision accuracy, and can be manipulated any time by the user.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\columnwidth]{fig/proxyArea.png}
  \caption{A user-defined scene proxy (\textbf{blue box}), delimiting the part of the game world for which collision information must be obtained.}\label{fig:proxyArea}
\end{figure}
\fi

\begin{figure}[ht]
  \subcaptionbox{Initial scene\label{fig:proxies_initial}}{\includegraphics[height=1.35in]{fig/proxy_1.png}}\hfill%
  \subcaptionbox{User-defined scene proxy\label{fig:proxies_defined}}{\includegraphics[height=1.35in]{fig/proxy_2.png}}\hfill%
  \subcaptionbox{Collision information within proxy\label{fig:proxies_evaluated}}{\includegraphics[height=1.35in]{fig/proxy_3.png}}%
  \caption{Definition of scene proxies to obtain collision information. The user delimits in which area of the original game scene (a) the cutscene will unfold via a scene proxy (b, \textbf{blue box}). Cine-AI then calculates collision information (c, \textbf{red boxes}) within that area.}
  \label{fig:proxies}
\end{figure}

Once the user has set up the scene proxies (Figure \ref{fig:proxies_defined}), \ProjectName{} calculates and serialises the collision data at design-time, enabling efficient collision avoidance during runtime. This calculation is repeated for each marker in the animation timeline, respecting the change of posture, position or orientation of the characters and objects in the scene (Figure \ref{fig:proxies_evaluated}).
%To this end, \ProjectName{} goes through each shot marker, evaluating the cinematic sequence at the exact time of the marker so that the objects being animated will get in their respective poses for that time. Evaluation is followed by calculating the collision data for each object within the proxy, which is repeated for each marker in the timeline.

\iffalse
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\columnwidth]{fig/proxyCalculation.png}
  \caption{Collision information (\textbf{red boxes}) calculated within the same scene proxy for two different markers, i.e. at two different times.}\label{fig:proxyCalc}
\end{figure}
\fi

%\ProjectName{} serializes the calculated collision data which can later be used while selecting camera positions as well as during the game while performing runtime collision avoidance.

\subsection{Selecting Cinematography Techniques}
\label{sec:system_selecting}

The user next initiates the simulation of all or specific shot markers (Supplementary Video, 01:40), yielding a set of cinematography techniques to be executed at the marker's time-step which (a) satisfy general cinematography principles, (b) imitate the target director, and (c) respect the user's settings. Here, we elaborate on the first sub-process in this simulation: the selection of suitable cinematography techniques (Table \ref{table:cinematography_techniques}) that satisfy these three requirements. To satisfy (a), the system filters the available techniques based on a general and shot-based ruleset, inspired by Kennedy and Mercer's Shotmaker system \citep{Kennedy}. It imitates the target director (b) by sampling one technique per category via the conditional probabilities determined from the director dataset (Section \ref{sec:system_data}). The sampled technique is then checked against the user-defined dramatisation and pace values (c). This process is repeated for each category (Positioning, Look, Tracking, FX;  Section~\ref{sec:data_categorisation}) in order, allowing to select e.g. a special effect based on the preceding tracking style.

%We use rejection sampling with technique sampling probabilities derived from the director style data and unsuitable techniques pruned based on hand-crafted rejection heuristics.

%based on rejection sampling. 

%A new camera behaviour, including the camera placement, angle, path, alignment and lens parameters is calculated based on the chosen techniques. 

%During the simulation, \ProjectName{} selects multiple cinematography techniques to use at the timestamp of the marker. We use rejection sampling with technique sampling probabilities derived from the director style data and unsuitable techniques pruned based on hand-crafted rejection heuristics. This procedure is performed consecutively for all categories, with the order as follows: positioning, look, tracking and fx. Following a specified order allows \ProjectName{} to consider the decisions given in the previous categories while choosing a cinematography technique for each category. This section explains the decision process and the reasoning behind it.

\subsubsection{General Rule Set Filtering}
%In order to implement both general and shot-based rule sets, we used a method inspired by the Shotmaker system of \citet{Kennedy}, where sets of rules direct the possible outcome cases, further eliminating the available cinematography techniques until only a handful is left. 
\ProjectName{} tries abides by a set of general cinematography rules, for instance: %about cinematography in order to realistically compose scenes and process shot sequences. The said rules are considered as the ABCs of film-making. 
\begin{description}
\item[Triangle Configuration:] If multiple subjects are within view, the camera should be focusing the middle of a triangle determined by the position of each subject \citep{Arijon}. 
\item[Rule of Thirds:] To create a natural balance in the shot composition, the subject is placed on top of the cross-over points between imaginary lines \citep{heiderich2012cinematography}. The visibility of the subject is always prioritised over the rule of thirds.
\item[Leading Subjects:] In a continuously moving sequence, a tracking camera should come to rest before its target stops.
%\item{Line of Action:} An imaginary line of action connecting the major subjects in the scene shall be used during the calculation of camera positions.
\end{description}

As first step in the selection of a set of cinematography techniques, each technique from a specific category is checked against the general rule set and filtered out if in violation. For instance, if the 3D geometry at a particular time, defined by the marker, does not permit a long distance shot, then techniques like long shot or master shot are removed. %Likewise, if it is not possible to focus on multiple targets defined by a single marker at a time, all targets except the first one defined by the user are eliminated from the target list.

%\ProjectName{} tries to enforce this rule on target subjects, whilst allowing users to control this process through parameters
Due to the interactive nature of games and the complexity of their 3D scenes, exactly abiding by all rules is often infeasible. To increase flexibility and customisability, \ProjectName{} allows users to tweak, or \enquote{bend}, each rule through a set of individual parameters. For instance, users can weaken or intensify the rule of thirds by adjusting  minimum and maximum shot distances, obedience thresholds, and visibility checking options. %to affect how strictly \ProjectName{} should behave during the decision process.%as well as the visibility checking options can be used

\subsubsection{Shot-based Rule Set Filtering} \ProjectName{} checks each technique that adheres to the general rule set against another set of rules designed to facilitate good shot compositions and avoid unwanted repetitions. In this second filtering process, the system incorporates information about the techniques decided for previous categories and preceding markers. The shot-based rule set includes the following key restrictions:

\begin{itemize}
  \item It is not possible to use consecutive fast zoom techniques (quick zoom, dolly zoom).
  \item It is not possible to transit a master shot into a close-up shot. The camera should not be covering distances larger than a user-defined threshold at a single transition.
  \item It is not possible to use consecutive slow motion effects.
  \item It is not possible to apply any tracking technique that affects the camera position if dolly zoom is to be used in the Look category of the current marker.
\end{itemize}
%These rules are mostly derived from well-accepted rules of cinematography. Additionally, they allow \ProjectName{} to avoid unwanted repetitions. 

\subsubsection{Director Data Sampling} \ProjectName{} finally samples one technique randomly from the remaining techniques based on the conditional probabilities calculated from the director data. This ensures that the selection yields techniques that are close to the target director's style, while affording stochastic variation if the user chooses to repeat the simulation.

%After the rule-based analysis of particular marker is done, \ProjectName{} is left with possible cinematography techniques to choose from. This is where the director data comes into play. A simple roulette selection function using the calculated probability of the techniques is performed in order to choose an available technique in the particular category.

Once a technique is selected, the dramatisation and pace values for the selected technique in the director's data is compared to the values designated by the user in the shot marker settings. If the selected technique does not fit the user's requirements, the sampling process is repeated until a suitable technique is found or a timeout is reached, in which case \ProjectName{} selects the default technique for the respective category (Table \ref{table:teccats}). The user can affect this process through threshold parameters, determining how strongly the marker's  dramatisation and pace values influence the selection. Based on these settings, the user can also skip the definition of dramatisation and pace values entirely. 

\iffalse
\begin{figure}[ht]
  \centering
  \includegraphics[width=4.0in]{fig/image_2021-02-17_171824.png}
  \caption{ User interface showing user choices for decision function to use as well as dramatisation and pace thresholds. }\label{fig:userChoiceDistribution}
\end{figure}
\fi

\subsection{Executing, Configuring and Validating the Camera Positioning}
\label{sec:system_executing}
The second simulation sub-process consists of configuring, executing and validating the previously selected camera positioning technique at the respective marker. It yields settings for camera placement, angle, path, alignment and lens; the \textit{look}, \textit{tracking} and \textit{FX} techniques do not need further refinement, and are simulated at runtime. 

%, determining the camera placement, angle, path, alignment and lens parameters at the respective marker. 

%So far, \ProjectName{} would have selected a cinematography technique from each category and obtained the collision data from the scene geometry. 

%Next step for \ProjectName{} to perform is to find a suitable camera position based on the technique selected from \textit{positioning} category, and fix any \textit{look}, \textit{tracking} as well as \textit{fx} behavior to be simulated in runtime. 

\subsubsection{Execute Technique.} For each user-designated shot marker, \ProjectName{} firstly positions the camera according to the selected technique. For instance, the implementation of the close-up shot (Table \ref{table:cinematography_techniques}) dictates that the camera must be within a meter from the target, while the master shot requires it to be sufficiently far away to capture the whole scene. 

\subsubsection{Validate Collisions.} After the camera is placed, the collision data from the scene proxies (Section \ref{sec:system_proxies}) is used to determine whether the placement is valid or not. In the latter case, \ProjectName{} tries a new positioning based on the randomisation properties of the executed technique until deemed valid, or a timeout is reached. 

\subsubsection{Validate Visibility.} As a last step, the camera is oriented towards the subject point to perform visibility checks with a raycasting algorithm: a virtual capsule travels from the camera position towards the target position to check if there are any objects blocking the path in between. If such an occluder is detected, \ProjectName{} falls back to finding a new camera position and restarts the cycle. In case of a timeout, \ProjectName{} returns to the technique selection sub-process.\\

%The execution cycle is only performed for the \textit{positioning} category. Due to the dynamic nature of the games it is possible to have a multitude of animation and sequence possibilities during a cutscene. Thus, continuous camera behaviors such as a quick zoom or handheld tracking techniques are executed in run-time. 

While our implementations of the cinematography techniques in Table \ref{table:cinematography_techniques} follow the most common cinematography rules \cite{Arijon}, we anticipate projects in which these rules yield undesirable outcomes. For instance, \ProjectName{} implements Mascelli's \citep{Mascelli} recommendation for close-up shots to depict the subject from the chest to above the head. However, this might not be fitting for non-humanoid characters. To provide more flexibility to its users, \ProjectName{} allows to customise each cinematography technique through a set of individual parameters. 
%. For instance, \citet{Mascelli} explains that a close-up shot depicts the subject from chest to above the head, which our system tries to achieve for all close-up shots. However, 

\iffalse
\begin{figure}[ht]
  \centering
  \includegraphics[width=2.8in]{fig/techniqueOptions.png}
  \caption{Example of per technique parameters exposed for users.}\label{fig:techniqueSettings}
\end{figure}
\fi 

\subsection{Storyboard}

%After all shot markers are simulated (Section \ref{sec:system_selecting} and \ref{sec:system_executing}), the outcome for each marker is presented as one node in the storyboard, a preview of the calculated shot

Motivated by the prevalence of storyboarding in movie pre-production, \ProjectName{} provides the users with a storyboard interface as the central control element to review and tweak the scene composition at design-time, without running the game (Supplementary Video, 01:45). \ProjectName{}'s storyboard visualises the composition (Section \ref{sec:system_selecting} and \ref{sec:system_executing}) by displaying each shot marker as an individual node in sequential order (Figure \ref{fig:storyboard_overview}), comprising various setting and a preview of the selected camera angles (Figure \ref{fig:storyboard_node}). Moreover, the storyboard summarises information on, and affords control of the imported director data, scene proxy settings and simulation parameters (Figure \ref{fig:storyboard_overview}, left panel). After tweaking e.g. the individual techniques and cinematography rules, users can re-simulate the results for one or more markers. Each marker has a lock option to protect it from changes while re-simulating. 

\begin{figure}[ht]
  \subcaptionbox{Storyboard overview\label{fig:storyboard_overview}}{\includegraphics[height=2.49in]{fig/storyboardwindow4.png}}\hfill%
  \subcaptionbox{Example storyboard node\label{fig:storyboard_node}}{\includegraphics[height=2.49in]{fig/storyboardnode2.png}}%
  \caption{Storyboard user interface. (a) Overview with each simulated shot marker, and (b) close-up view of a shot marker's parameters, selected cinematography techniques and a preview of the marker}
\end{figure}

Once the user is satisfied and confirms the cutscene composition, \ProjectName{} serialises all shot data in Unity asset files for use at runtime. It comprises e.g. target subjects, locations, the selected cinematography techniques with custom settings, and the simulated camera positioning. Our data representation is derived from the FILM language \citep{Charles}, a processing language designed to characterise the behaviour of camera motion within any given 3D world geometry. %Having done most of the heavy work done at design-time, \ProjectName{} can process the camera behaviour at runtime with very low resource requirements. 

% After the desired settings are ready, users can start simulating each marker in their cutscene using the storyboard window. The simulation will perform the steps mentioned in the previous sections, leading to a camera placement and a clear view of the subject. The final camera view will be rendered as a preview texture which can be seen below the nodes for each marker in the storyboard window.

%Additionally, storyboard window allows users to re-simulate particular markers if the results are not as desired. Each marker can be re-simulated individually. Moreover, users can lock specific nodes they prefer to keep in the final composition. Thus, when a full re-simulation is executed, locked nodes will not be affected and will preserve their previous simulation data.


%\section{Storing Data and High Level Language}

%Once a final scene composition is achieved, all the markers will have been processed with respect to rule sets, cinematography technique decisions and their implementations. Since all of the said operations will be done in design-time, it is eligible to create an arbitrary language that the system can use to process this information in runtime.

%\citet{Charles} introduces the FILM language, a processing language designed to characterize the behaviour of camera motion within any given 3D world geometry. The FILM language consists of variables for a given scene, such as unique identifiers, participants, scene type and shot lists. It also describes details about the shots including target subjects, constraints, locations and transitions. Similarly, a simple representation of such a high level system was defined, by keeping our scene composition data in serializable objects for easy distribution. In the case of Unity game engine we are using, scriptable objects, classes that can contain any type of information and are distributable as asset files were used to hold the expressions of such arbitrary language. In \ProjectName{}, scriptable objects hold all the information about all the markers, including the selected cinematography techniques, implementation details of the said techniques and simulated data about the camera orientation. Therefore, all data related to the simulation process is stored in an asset file, completely in design-time. By having most of the heavy work done before the runtime, \ProjectName{} can simply look-up this file from memory and process the camera behaviour without any additional performance costs during runtime.

%\begin{figure}[H]
%  \centering
%  \includegraphics[width=3.0in]{fig/scriptableObject.png}
%  \caption{Scriptable object showing the selected %techniques and information about the target %marker.}\label{fig:scriptableObject}
%\end{figure}
%
\subsection{Runtime Execution}

The storyboarding completes \ProjectName{}'s design-time workflow; to play the in-game cutscene at runtime, the system listens to events fired as each shot marker is hit over time, and executes the corresponding cinematography techniques (Supplementary Video, 02:30). Although almost all required data is calculated at design-time, the system must still perform some operations at runtime to realise a crucial feature: its applicability to dynamic cutscenes. In such scenes, the behaviour of e.g. objects, animations and non-player characters (NPCs) can vary based on the preceding, player-induced game state; an NPC for instance might walk to different places in the scene, depending on the player's previous choices. 

Pre-calculating animations that reach across multiple frames at design-time is only feasible for static cutscenes. This applies to all techniques from the \textit{look}, \textit{tracking} and \textit{FX} categories, and \ProjectName{} consequently executes those at runtime. The potentially dynamic nature of the cutscene also implies that the 3D geometry might change in ways unanticipated during the design-time collision detection via scene proxies, thus necessitating runtime collision avoidance. If the camera penetrates an object, \ProjectName{} performs Haigh-Hutchinson’s algorithm \citep{Haigh} to move the camera along the object's surface. %whenever the camera detects a collision during the cutscene, it will slide on the surface of the collided mesh with an angle perpendicular to the surface's normal.
These runtime calculations require some additional computational resources, but enable the user to create only a single cutscene composition through \ProjectName{}, which can then adapt flexibly to the game at runtime.

%We motivate this design decision from two angles.
% to better respond to dynamic changes in the game scene.
%, e.g. player-induced variations in the game-state immediately before the cutscene.

%here, we briefly explain the system's runtime processing for the in-game cutscene. 

%As the users' cutscenes play, \ProjectName{} listens to events fired when each time a shot marker is hit, executing the cinematography techniques during the marker's timestamp. However, even though almost all the data related to the camera motion is calculated in design-time, performing some of the operations in runtime is still necessary to allow better responses towards dynamic changes in the scene. This section explains the runtime aspect of \ProjectName{}.

%For instance, the dolly zoom technique (Table \ref{table:cinematography_techniques}) requires moving the camera away from the subject while simultaneously decreasing the camera's field of view. However, 

\iffalse
\begin{figure}[H]
  \centering
  \includegraphics[width=4.0in]{fig/colavod.png}

  \caption{\textcolor{red}{Remove or replace with more illustrative image? }Camera performing line-casting for collision avoidance, detecting a wall behind and rejecting to move further towards back.}\label{fig:scriptableObject}
\end{figure}
\fi
